Entity, Relation, and Event Extraction with Contextualized Span Representations

We examine the capabilities of a unified, multi-task framework for three information extraction tasks: named entity recognition, relation extraction, and event extraction. Our framework (called DyGIE++) accomplishes all tasks by enumerating, refining, and scoring text spans designed to capture local (within-sentence) and global (cross-sentence) context. Our framework achieves state-of-the-art results across all tasks, on four datasets from a variety of domains. We perform experiments comparing different techniques to construct span representations. Contextualized embeddings like BERT perform well at capturing relationships among entities in the same or adjacent sentences, while dynamic span graph updates model long-range cross-sentence relationships. For instance, propagating span representations via predicted coreference links can enable the model to disambiguate challenging entity mentions. Our code is publicly available at https://github.com/dwadden/dygiepp and can be easily adapted for new tasks or datasets.

==> event-prop.tex <==
\section{Graph Propagation} \label{sec:event_graph}

\newcommand{\trig}{\bh_i}
\newcommand{\argu}{\bg_j}
\newcommand{\simil}{\bV_A^t(i, j)}
\newcommand{\similprime}{\bV_A^{t'}(i, j)}
\newcommand{\updateArgTrig}{\bu^t_{A \to T}(i)}
\newcommand{\gateArgTrig}{f_{A \to T}^t(i)}
\newcommand{\weightArgTrig}{\bW_{A \to T}}
\newcommand{\updateTrigArg}{\bu^t_{T \to A}(j)}
\newcommand{\gateTrigArg}{f_{T \to A}^t(j)}
\newcommand{\weightTrigArg}{\bW_{T \to A}}

We follow similar relation and coreference interactions described in \citet{luan2019general}, and extend them to incorporate events. Here, we detail the propagation step to incorporate global context for events because it consists of two types of nodes in the graph: triggers and arguments, whereas relations and coreferences include single-type nodes.
 
The intuition behind the event graph is to provide each trigger with information about its potential arguments, and each potential argument with information about triggers for the events in which it might participate.\footnote{Event propagation is a somewhat different idea from \cite{Sha2018JointlyEE}, who model argument-argument interactions using a learned tensor. We experimented with adding a similar tensor to our architecture, but did not see any clear performance improvements.} The event propagations are different from relation and coreference updates because there are two types of nodes: triggers and arguments. 

%$\trig$ for each token candidate $\bd_i$ by simply repeating its token embedding twice and concatenating a span width embedding.

The model iterates between updating the triggers based on the representations of their likely arguments, and updating the arguments based on the representations of their likely triggers. More formally, denote the number of possible semantic roles played by an event argument (i.e. the number of argument labels) as $L_A$,  $B_T$ as the trigger beam, and  $B_A$ as the argument beam. 
For each trigger $\trig^t \in B_T$ and argument $\argu^t \in B_A$, the model computes the similarity vector $\simil$ as the current trigger/argument score predicted through a feedforward neural network. % by feeding $[\trig^t, \argu^t, \bC]$ through a feedforward neural network (FFNN), where $\bC$ is the BERT class label for the sentence containing $\trig^t$ and $\argu^t$. 
The $k^{th}$ element of $\simil$ scores how likely it is that argument $\argu$ plays role $k$ in the event triggered by $\trig$. 

Extending Equation~\ref{eq:prop}, the model  updates the trigger $\trig$ by taking an average of the candidate argument embeddings, weighted by the likelihood that each candidate plays a role in the event:
\begin{equation} \label{eqn:trigger_update}
    \updateArgTrig = \sum_{j \in B_A} \bA_{A \to T} f(\simil) \odot \argu^t,
\end{equation}
where $\bA_{A \to T} \in \reals^{d \times L_A}$ is a learned projection matrix, $f$ is a ReLU function, and $\odot$ is an elementwise product. Then, the model computes a gate determining how much of the update from (\ref{eqn:trigger_update}) to apply to the trigger embedding:
\begin{equation} \label{eqn:gate}
\gateArgTrig = \sigma \left(\weightArgTrig [\trig^t, \updateArgTrig] \right),
\end{equation}
where $\weightArgTrig \in \reals^{2d \times d}$ is a learned projection matrix and $\sigma$ is the logistic sigmoid function. Finally, the updated trigger embeddings are computed as follows:
\begin{equation} \label{eqn:new_span}
    \trig^{t+1} = \gateArgTrig \odot \trig^t + (1 - \gateArgTrig) \odot  \updateArgTrig.
\end{equation}

Similarly, an update for argument span $\argu$ is computed through messages $\updateTrigArg$ as a weighted average over the trigger spans similar to Equation~\ref{eqn:trigger_update}, with a new trainable matrix $\bA_{T \to A}$: % the learned  The learned projection matrix in this s

\begin{equation}
    \updateTrigArg = \sum_{i \in B_T} \bA_{T \to A} f(\similprime) \odot \trig^{t+1}, 
\end{equation}
where $\similprime = \text{FFNN}([\trig^{t+1}, \argu^t])$ is recomputed trigger/argument score.  

Next we compute the argument update gate

\begin{equation}
    \gateTrigArg = \sigma \left( \weightTrigArg [\argu, \updateTrigArg] \right)
\end{equation}

where $\weightTrigArg \in \reals^{2d \times d}$ is another learned projection matrix. Finally, the updated argument embeddings are computed like

\begin{equation}
    \argu^{t+1} = \gateTrigArg \odot \argu^t + (1 - \gateTrigArg) \odot \updateTrigArg
\end{equation}

This process represents one iteration of event graph propagation. The outputs of the graph propagation are contextualized trigger and argument representations. When event propagation is performed, the final trigger scorer takes the contextualized surrogate spans $\trig$ as input rather than the original token embeddings $\bd_i$.

\newcommand{\similArgTrig}{\bS_{A \to T}(i, j)}
\newcommand{\similTrigArg}{\bS_{T \to A}(i, j)}

The similarity matrices are

\begin{equation}
    \similArgTrig =  \bA_{A \to T} f(\simil)
\end{equation}

and

\begin{equation}
    \similTrigArg =  \bA_{T \to A} f(\simil)
\end{equation}

Then the updates are 

\begin{equation} \label{eqn:trigger_update}
    \updateArgTrig = \sum_{j \in B_A} \similTrigArg \odot \argu^t,
\end{equation}

\begin{equation}
    \updateTrigArg = \sum_{i \in B_T} \similArgTrig \odot \trig^{t+1}, 
\end{equation}

==> tables/ablation_bert_relprop.tex <==
\begin{table*}[]
  \begin{tabular}{|l|l|l|l|}
    \hline
    Relation ACE  BERT no finetuning - LSTM dev set & 0    & 1    & 2    \\ \hline
    BERT 1 Sentence                                 & 59.3 & 59.8 & 60.7 \\ \hline
    Bert 3 Sentences                                & 60.6 & 60.2 & 61.3 \\ \hline
    BERT 5 Sentences                                & 60.3 & 59.7 & 61.9 \\ \hline
  \end{tabular}
  \caption{\luanyi{We really need a figure to show how performances change with number of sentences on BERT. The number of iteration may not be that important since we have shown that in our last paper. Maybe pick the best number for each row and do a plot comparing finetuning bert and not finetuning bert.}}
\end{table*}
